Model-Guided Network with Cluster-Based Operators for Spatio-Spectral Super-Resolution

This paper addresses the problem of reconstructing a high-resolution hyperspectral image from a low-resolution multispectral observation. While spatial super-resolution and spectral super-resolution have been extensively studied, joint spatio-spectral super-resolution remains relatively explored. We propose an end-to-end model-driven framework that explicitly decomposes the joint spatio-spectral super-resolution problem into spatial super-resolution, spectral super-resolution and fusion tasks. Each sub-task is addressed by unfolding a variational-based approach, where the operators involved in the proximal gradient iterative scheme are replaced with tailored learnable modules. In particular, we design an upsampling operator for spatial super-resolution based on classical back-projection algorithms, adapted to handle arbitrary scaling factors. Spectral reconstruction is performed using learnable cluster-based upsampling and downsampling operators. For image fusion, we integrate low-frequency estimation and high-frequency injection modules to combine the spatial and spectral information from spatial super-resolution and spectral super-resolution outputs. Additionally, we introduce an efficient nonlocal post-processing step that leverages image self-similarity by combining a multi-head attention mechanism with residual connections. Extensive evaluations on several datasets and sampling factors demonstrate the effectiveness of our approach. The source code will be available at https://github.com/TAMI-UIB/JSSUNet

==> fig_results_CAVE.tex <==
% Define the dimensions outside the \spyimage command


% Define the \spyimage command with unique-length names
\newcommand{\spyimageCAVE}[2][0.22\linewidth]{%
  % Set the dimensions within the command
  \setlength{\spyimagewidth}{#1}
  \setlength{\spyimageheight}{\spyimagewidth}
  \begin{tikzpicture}[spy using outlines={rectangle, magnification=2, size=0.4\spyimagewidth, connect spies,color=white}]
    % Insert the image
    \node[inner sep=0pt, anchor=south west] (image) at (0,0) {\includegraphics[width=\spyimagewidth]{#2}};
    % Coordinates of the zoom point
    \coordinate (spy point) at (0.5\spyimagewidth , 0.75\spyimageheight );
    % Coordinates where the zoom will appear
    \coordinate (spy node) at (0.2\spyimagewidth, 0.2\spyimageheight);
    % Apply the spy command
    \spy on (spy point) in node at (spy node);
  \end{tikzpicture}%
}
% In the document body

\begin{figure*}[t]
    \centering
\begin{tabular}{c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em}}
    \spyimageCAVE{CAVE_gt.png} &
    \spyimageCAVE{CAVE_AWAN-SSPSR.png}  &
    \spyimageCAVE{CAVE_SSPSR-AWAN.png}  &
    \spyimageCAVE{CAVE_SSPSR-AWAN-Fusformer.png}  \\


    GT & AWAN-SSPSR & SPSSR-AWAN & SSPSR-AWAN-Fusformer \\

    &
    \spyimageCAVE{CAVE_US3RN.png}  &
    \spyimageCAVE{CAVE_SSFIN.png}  &
    \spyimageCAVE{CAVE_Ours.png}  \\

 & US3RN & SSFIN & Ours \\

\end{tabular}
    \caption{Visual comparison on CAVE test set for sampling of 2. For each method, the high-resolution result is displayed. Our method achieves sharper contours and correctly preserves color, while the other methods produce artifacts in the outlines of the jelly beans.}
    \label{fig:cave}
\end{figure*}


==> fig_results_Pavia.tex <==
% Define the dimensions outside the \spyimage command


% Define the \spyimage command with unique-length names
\renewcommand{\spyimageCAVE}[2][0.22\linewidth]{%
  % Set the dimensions within the command
  \setlength{\spyimagewidth}{#1}
  \setlength{\spyimageheight}{\spyimagewidth}
  \begin{tikzpicture}[spy using outlines={rectangle, magnification=2, size=0.5\spyimagewidth, connect spies,color=white}]
    % Insert the image
    \node[inner sep=0pt, anchor=south west] (image) at (0,0) {\includegraphics[width=\spyimagewidth]{#2}};
    % Coordinates of the zoom point
    \coordinate (spy point) at (0.35\spyimagewidth , 0.15\spyimagewidth );
    % Coordinates where the zoom will appear
    \coordinate (spy node) at (0.25\spyimagewidth, 0.75\spyimageheight);
    % Apply the spy command
    \spy on (spy point) in node at (spy node);
  \end{tikzpicture}%
}
% In the document body

\begin{figure*}[t]
    \centering
\begin{tabular}{c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em}}
    \spyimageCAVE{Pavia_gt.png} &
    \spyimageCAVE{Pavia_AWAN-SSPSR.png}  &
    \spyimageCAVE{Pavia_SSPSR-AWAN.png}  &
    \spyimageCAVE{Pavia_SSPSR-AWAN-Fusformer.png}  \\


    GT & AWAN-SSPSR & SPSSR-AWAN & SSPSR-AWAN-Fusformer \\

    &
    \spyimageCAVE{Pavia_US3RN.png}  &
    \spyimageCAVE{Pavia_SSFIN.png}  &
    \spyimageCAVE{Pavia_Ours.png}  \\

 & US3RN & SSFIN & Ours \\

\end{tabular}
    \caption{Visual comparison on Pavia test set for sampling of 2. For each method, the high-resolution result is displayed. Our method produces the most vivid colors as it is evidenced in the red car of the highlighted area. At the same time, we correctly preserve the image geometry, while the other approaches yield smoother results.}
    \label{fig:pavia}
\end{figure*}


==> fig_results_ntire2020_2.tex <==
% Define the dimensions outside the \spyimage command


% Define the \spyimage command with unique-length names
\newcommand{\spyeimagentire}[2][0.22\linewidth]{%
  % Set the dimensions within the command
  \setlength{\spyimagewidth}{#1}
  \setlength{\spyimageheight}{\spyimagewidth}
  \begin{tikzpicture}[spy using outlines={rectangle, magnification=3, size=0.5\spyimagewidth, connect spies,color=white}]
    % Insert the image
    \node[inner sep=0pt, anchor=south west] (image) at (0,0) {\includegraphics[width=\spyimagewidth,trim={0 1.1cm 0 0},clip]{#2}};
    % Coordinates of the zoom point
    \coordinate (spy point) at (0.32\spyimagewidth , 0.795\spyimagewidth );
    % Coordinates where the zoom will appear
    \coordinate (spy node) at (0.25\spyimagewidth, 0.25\spyimageheight);
    % Apply the spy command
    \spy on (spy point) in node at (spy node);
  \end{tikzpicture}%
}


\begin{figure*}[t]
    \centering
\begin{tabular}{c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em} c@{\hskip 0.2em}}
    \spyeimagentire{ntire2020_gt.png} &
    \spyeimagentire{ntire2020_AWAN-SSPSR.png}  &
    \spyeimagentire{ntire2020_SSPSR-AWAN.png}  &
    \spyeimagentire{ntire2020_SSPSR-AWAN-Fusformer.png}  \\

    GT & AWAN-SSPSR & SPSSR-AWAN & SSPSR-AWAN-Fusformer \\

    &
    \spyeimagentire{ntire2020_US3RN.png}  &
    \spyeimagentire{ntire2020_SSFIN.png}  &
    \spyeimagentire{ntire2020_Ours.png}  \\

 & US3RN & SSFIN & Ours \\

\end{tabular}
    \caption{Visual comparison on NTIRE2020 test set for sampling of 8. For each method, the high-resolution result is displayed. As it can be observed in the highlighted area, US3RN and SSFIN are unable to recover chromaticity and fail to reconstruct the geometry. Non-specific SSSR methods offer a better spectral retrieval, but provide smooth solutions. In contrast, our method achieves superior geometry reconstruction and color preservation.}
    \label{fig:ntire2020}
\end{figure*}

